ReCycle: Resilient Training of Large DNNs using Pipeline Adaptation

Training large Deep Neural Network (DNN) models requires thousands of GPUs over the course of several days or weeks. At this scale, failures are frequent and can have a big impact on training throughput. Utilizing spare GPU servers to mitigate performance loss becomes increasingly costly as model sizes grow. ReCycle is a system designed for efficient DNN training in the presence of failures, without relying on spare servers. It exploits the inherent functional redundancy in distributed training systems -- where servers across data-parallel groups store the same model parameters -- and pipeline schedule bubbles within each data-parallel group. When servers fails, ReCycle dynamically re-routes micro-batches to data-parallel peers, allowing for uninterrupted training despite multiple failures. However, this re-routing can create imbalances across pipeline stages, leading to reduced training throughput. To address this, ReCycle introduces two key optimizations that ensure re-routed micro-batches are processed within the original pipeline schedule's bubbles. First, it decouples the backward pass into two phases: one for computing gradients for the input and another for calculating gradients for the parameters. Second, it avoids synchronization across pipeline stages by staggering the optimizer step. Together, these optimizations enable adaptive pipeline schedules that minimize or even eliminate training throughput degradation during failures. We describe a prototype for ReCycle and show that it achieves high training throughput under multiple failures, outperforming recent proposals for fault-tolerant training such as Oobleck and Bamboo by up to $1.46\times$ and $1.64\times$, respectively.

==> sections/planner_backup.tex <==
\section{\NAME Design}\label{sec:design}

%\NAME realizes the benefits of \textit{Adaptive Pipelining}, \textit{Decoupled BackProp}, and the \textit{Staggered Optimizer} in an end-to-end training system.
%\myzhao{If we have space, a figure that shows these components will be useful}
%As shown in Figure XX, \NAME consists of three critical components, a \textit{Profiler}, \textit{Executor}, and critically a \textit{Planner}.
%We begin by walking through how \NAME leverages these components to manage and ensure the resiliency of the training job.
%Section~\ref{sec:planner} then describes how the \textit{Planner} leverages the key techniques to generate efficient training schedules even under failures.

\subsection{System Overview}\label{sec:design_overview}
\NAME consists of three components, a \textit{Profiler}, \textit{Executor}, and critically a \textit{Planner}.

\noindent\textbf{Profiler:}
When a large training job is first submitted, 
\NAME runs a short profiling job to collected key performance statistics such as the average micro batch latency for the forward and backward passes, memory requirements for activations and gradients, and inter-node communication bandwidth. \myzhao{check me} The profiling job executes a small number of training iterations, 100 by default, and typically takes a few minutes. 
The \textit{Profiler} aggregates the collected statistics for use by the \textit{Planner}.

\noindent\textbf{Planner.} The \textit{Planner} generates near optimal schedules for the training job under various failure scenarios. \christos{check} It uses dynamic programming (DP) and mixed integer linear program (MILP) formulations that implement the \NAME {sec:system}.  We generate a pipeline schedule for each \textit{number} of tolerated simultaneous failures. Each plan is agnostic to which specific worker(s) fail. It encodes the specific pipeline schedule including micro-batch assignment, the order of forward and backward tasks (e.g., \textit{ForwardPass}, \textit{BackwardWeightPass}), and the communication plan (e.g., \textit{RecvActiv}, \textit{SendGrad}, etc.).
The set of  plans is stored in distributed fault-tolerant storage (e.g., \textit{etcd}) to be accessed by \textit{Executors} during runtime.

By default, we generate up to $DP-1$ plans, which accounts for $DP-1$ simultaneous failures that \NAME can always handle. Since \NAME can probabilistically sustain many more failures, we generate plans for up to a user-defined fault tolerance threshold. The \textit{Planner} runs relatively quickly, $\approx50$ minutes to generate plans for up to 24 failures for a cluster of 1700 GPUs. Nevertheless, the training job can begin training in parallel as most plans will not be needed immediately. 

\noindent\textbf{Executors.}
\NAME runs a \textit{Executor} in each GPU node which is responsible for 
executing the training plan for the node. A centralized \textit{Coordinator} manages the overall training job by specifying the correct execution plan for each \textit{Executor}.
The \textit{Coordinator} continuously monitors the health of \textit{Executors}.
Upon detecting a failure, it looks up the execution plan for the number of currently failed workers and informs remaining \textit{Executors} to resume execution according to the new plan. Execution restarts from the iteration during which the failure was detected with no need for parameter re-shuffling across nodes. Restoring a checkpoint from remote storage is only necessary for failures with long detection intervals.  The \textit{Coordinator} itself is made fault-tolerant via active replication.

\subsection{\NAME Planner}\label{sec:planner}
Given the cluster configuration, training job, \textit{Profiler} statistics, and set of failed workers, the \textit{Planner} calculates a valid pipeline execution schedule that minimizes the overall training iteration latency using the fault-free workers. the \textit{Planner} uses  two phases, \textit{Normalization} followed by \textit{Solution}.

\NAME generates a execution plan for a given \textit{number} of failures, regardless of \textit{which} worker(s) fails, a solving ILP problems for the combinatorial number of possible failure locations is intractable.
The first phase \textit{normalizes} a specific number of failures by migrating failed nodes to a pre-determined and ideal set of locations within the pipeline schedule.
%Thus, regardless of the initial worker failure locations, \NAME first re-orders the 3D parallelism groups to ensure that the second (and expensive) phase only needs to generate one solution for a given number of failures.
For example, if \textit{any} single node fails in the example in Figure~\ref{fig:recovery-in-recycle}, \NAME will always swap the node with an ideal location, e.g. $W_{2\_3}$.  The \textit{Planner} generates a mapping of the ideal migration locations for each possible number of simultaneous failures.  
The \textit{Solution Phase} leverages an MILP to derive an optimized schedule for each normalized case. \christos{maybe 1 sentence on how to project back to the specific failure case? the naive approach requires a lot of parameter re-shuffling which we claim we don't do much}


\subsubsection{Normalization Phase}\label{sec:normalization-phase}
The intuition behind the Normalization Phase is to ensure that a) failures are distributed across different peer groups \myzhao{todo: make sure term is consistent elsewhere} and b) move failures to pipeline stages with more bubbles.
Distributing failures across peer groups to both maximizes fault tolerance (minimizing the probability of losing an entire peer group as in Figure~\ref{fig:not-recoverable}) and ensures that extra work is across different peer groups, avoiding bottlenecks that can impede overall system performance.
Meanwhile, increasing the number of bubbles maximizes the opportunity to hide overheads that applying the techniques in Section~\ref{sec:system} can introduce.
\christos{my suggestions is two add 2-3 sentences here and move the rest of his to the appendex (icnlduing the algorithm. The additional text here should say why DP (as opposed to something esle and the cost function heuristic it optimizes}

\noindent\textbf{DP Formulation.}
%Intuitively, the Normalization Phase migrates failures across peer groups and deeper into the pipeline (i.e., to stages with more bubbles).
To formalize this intuition, we leverage a dynamic programming (DP) solution that determines the ideal location to migrate faults to given a number of failures as shown in Algorithm~\ref{alg:normalization}.

\input{figures/dp-alg}

Given the total number of failures to handle, $F$, and the total number of pipeline stages within a data parallel pipeline, $N$, the DP algorithm returns a list $R$ of length $N$, such that $\Sigma_{i} R[i]=F$.
Each index $R[i]$ specifies the ideal number of failures that is assigned to pipeline stage $i$ across all data parallel pipelines; the specific pipeline assignment does not affect performance and can be arbitrary.
For example, if $R[3]=2$ for the example in Figure~\ref{fig:not-recoverable}, the ideal migration would be to swap the failed nodes with any two nodes in stage $3$, for example $W_{0\_3}$ and $W_{2\_3}$.

For each DP step, $C[i][f]$ represents the total cost, in terms of bubbles used, to handle $f$ failures at all stages between $0$ and $i$. 
Meanwhile, each $A[i][f]$ contains a list that denotes the portion of the $f$ failures assigned to each stage from $0$ to $i$, as described for $R$ -- in other words $len(A[i][f]) == i+1$.
Each DP step uses a recurrence relation that aims to minimize the cost of handling $f$ failures within the first $i$ pipeline stages across all of the data parallel pipelines, while $A[i][f]$ denotes the assignment of failures that achieves this cost.
The ideal assignment to handle $F$ failures across all workers is simply $R = A[N-1][F]$.

To estimate the cost, $cost(i, x)$ is a function that returns the extra bubbles used to handle the extra micro batches from $x$ failures in the $i$-th stage (i.e., peer group).
While we can use the MILP described in Section~\ref{sec:solution} to estimate the cost, the \textit{Planner} can also rely on a heuristic to estimate the cost in order to avoid longer solve times (as Algorithm~\ref{alg:normalization} requires $O(NF)$ calls to the cost function).
The heuristic captures the benefit of the techniques described in Section~\ref{sec:system}.
It creates a pipeline schedule that is similar to 1F1B, except that the heuristic's 1F1B backward pass only schedules $B_{input}$.
Then, when there exists a gap (both in terms of time and memory) that is able to fit $B_{weight}$ (or the $F$ and $B_{input}$ stages are exhausted), $B_{weight}$ operations are scheduled opportunistically.
%Surrogate micro-batches are 

Thus, upon any detected failure, the \textit{Coordinator} will first perform the migration strategy to normalize the failed nodes according to Algorithm~\ref{alg:normalization} before proceeding with the optimized execution plan.
\myzhao{@swapnil, i'm assuming this is what would need to happen? If so, what explicitly would this do? shuffle weights to necessary workers? anything else?}

\subsubsection{Phase 2: Solution Phase}\label{sec:solution}
%In the second phase, the \textit{Planner} uses an MILP to determine the optimal execution plan given a number of worker failures.
Next, the \textit{Planner} uses the normalized failure locations and the profiled statistics as inputs to an MILP that finds an optimized ordering of training operations. %which the \textit{Planner} converts to an execution plan.
%Here, we describe the MILP formulation, which can be solved using an off-the-shelf MILP solver such as Gurobi.
%\myzhao{Ok, i tried my best to decipher the math, but swapnil please check me on all of this...}

\noindent\textbf{Notation.}
An operation within a training iteration can be explicitly identified across workers using a 5-tuple $(i, j, k, c, k_s)$.
$i$ represents the pipeline stage within each data parallel pipeline, while $k$ represents the operation's original data parallel pipeline (prior to failures).
$j$ is the micro batch ID in the training iteration.
$c$ identifies the different operations for each micro batch, $c \in \{F, B_input, B_weight\}$.
Finally, $k_s$ denotes the \textit{surrogate} pipeline in the event that a micro batch \textit{originally} intended for $k$ runs on $k_s$ (note that $k$ can equal $k_s$).
For example, a micro batch originally intended to execute on $W_{2\_3}$, but was re-routed to a surrogate $W_{1\_3}$ in Figure~\ref{fig:recovery-in-recycle}, would have $i=3$, $k=2$, and $k_s=1$.
Thus, $(i, k_s)$ uniquely identifies the worker for a given operation.

\noindent\textbf{Inputs.}
The MILP takes as input the micro batch to worker assignments in an iteration.
Specifically, the \textit{Planner} takes the normalized failure locations and assigns all micro batches corresponding to failed workers evenly across surrogate workers within the same peer group, alongside the original (non-surrogate) micro batches.
Thus, the \textit{Planner} produces a binary mapping $S_{i,j,k}^{k_s} \in \{ 0, 1 \}$, which indicates if a micro batch $(i, j, k)$ should be executed on pipeline $k_s$.
Note that $S_{i,j,k}^{k}=1$ if the micro batch executes on the original pipeline.
We ensure that each operation is assigned only one pipeline, i.e., \( \sum_{\substack{k_s}} S_{i,j,k}^{k_s} = 1 \).
%Note that $k$ can equal $k_s$.

The MILP also takes as input profiled statistics.
First, $T_c$ represents the computational time for each operation $c$.
$T_{comm}$ represents the communication latency to send activations or gradients across workers\footnote{We use a single value as activations and gradients are the same size.  \myzhao{Double check me here}}.
Next, the MILP requires the \textit{change} in memory utilization on worker $(i, k, k_s)$ caused by executing an operation $(i, j, k, c, k_s)$ as \(\Delta M_{i,j,k,c}^{k_s}\).

\begin{equation*}
\Delta M_{i,j,k,c}^{k_s} =
\begin{cases}
    A_{B} & \text{, if } c=F \text{ and  } S_{i,j,k}^{k_s} = 1 \\
    A_B - A_{B_{Input}} & \text{, if } c=B_{Input} \text{ and } S_{i,j,k}^{k_s} = 1 \\
    -A_{B_{Weight}} & \text{, if } c=B_{Weight} \text{ and } S_{i,j,k}^{k_s} = 1 \\
    0 & \text{, otherwise}
\end{cases}
\end{equation*}

Here, \(A_B\) is the profiled size of activation stored at the end of forward pass.
$A_{B_{input}}$ and \(A_{B_{Weight}}\) is size of the activation stored at the end of backward-input and backward-weight pass, respectively.
Upon completion of backward-input pass and backward-weight pass, we free activation \(A_{B_{Input}}\) and \(A_{B_{Weight}}\) respectively.

\noindent\textbf{Variables.}
The goal of the MILP is to identify the exact ordering of operations, which can be used to generate a pipeline schedule.
To do this, we introduce an ordering variable $O_{(i,j,k,c,k_s)\rightarrow(i^\prime,j^\prime,k^\prime,c^\prime,k_s^{\prime})} \in \{ 0, 1 \}$ between each pair of operations $(i, j, k, c, k_s)$ and $(i^\prime, j^\prime,k^\prime,c^\prime,k_s^{\prime})$.
Each variable is 1 if  $(i^\prime, j^\prime,k^\prime,c^\prime,k_s^{\prime})$ is scheduled any time after $(i, j, k, c, k_s)$ and 0 otherwise.
Ordering is only required within a stage, and between computation phases of same micro batch (e.g., between the $F$ and $B_{input}$ pass).
Finally, we define the set of variables \(E_{i,j,k,c}^{k_s}\) as the ending time of operation \( (i,j,k,c,k_s) \).

\noindent\textbf{Objective.}
The goal of the MILP is to minimize the makespan of a single training iteration (which is repeated throughout the training process).
This can be done by determining the sequence and time of operations through the training pipeline via the sets of variables $O$ and $E$.
This objective can thus be formulated as: 
\myzhao{i think there was a typo in the original objective, so check me.}

\begin{equation}
    \min_{\substack{O, E}} \qquad \max_{\substack{i,j,k,k_s}} E_{i,j,k,B_{Weight}}^{k_s} 
\label{eq:ilp-optim-target}
\end{equation}

Here, $\max_{i,j,k,k_s} E_{i,j,k,B_{Weight}}^{k_s}$ represents the end time of the \textit{last} operation in the iteration, representing the makespan.

\noindent\textbf{Constraints.}
The constraints applied to the objective are the following.

\noindent\textit{Cross-Stage Dependencies.}
\begin{equation}
E_{i,j,k,F}^{k_s} \ge 
    S_{i,j,k}^{k_s} \times 
        (\sum_{\hat{k}} (E_{i-1,j,k,F}^{\hat{k}} \times S_{i-1,j,k}^{\hat{k}}) \\ + T_{comm} + T_{F})
\label{eq:ilp-cross-stage-dep-forward}
\end{equation}

% Backward-Input Pass
\begin{equation}
    \begin{multlined}
    E_{i,j,k,B_{Input}}^{k_s} \ge 
        S_{i,j,k}^{k_s} \times
            (\sum_{\hat{k}} (E_{i+1,j,k,B_{Input}}^{\hat{k}} \times S_{i+1,j,k}^{\hat{k}}) \\ + T_{comm} + T_{B_{Input}})
    \end{multlined}
\label{eq:ilp-cross-stage-dep-backward}
\end{equation}

Equation~\ref{eq:ilp-cross-stage-dep-forward} specifies the dependency of a given micro batch's forward pass on previous pipeline stages (e.g., stage 0 must execute before stage 1).
Similarly, Equation~\ref{eq:ilp-cross-stage-dep-backward} specifies the reverse dependency for the backward pass (e.g., stage 1 must execute before stage 0).

\noindent\textit{Same-Stage Dependencies.}
\begin{equation}
E_{i,j,k,B_{Weight}}^{k_s} \ge 
    S_{i,j,k}^{k_s} \times (E_{i,j,k,B_{Input}}^{k_s} + T_{B_{Weight}})
\label{eq:ilp-same-stage-dep}
\end{equation}

Equation~\ref{eq:ilp-same-stage-dep} allows the MILP to reason about \textit{Decoupled BackProp}, specifying that $B_{input}$ must precede $B_{weight}$ for a given micro batch within a worker.

\noindent\textit{No Overlapping Computations.}
\begin{equation}
    \begin{multlined}
    E_{i,j^\prime,k^{\prime},c^\prime}^{k_s^{\prime}} \ge 
    E_{i,j,k,c}^{k_s^{\prime}} + T_{c^\prime} - \\ \infty (1 - S_{i,j,k}^{k_s^{\prime}} \times S_{i,j^\prime,k^\prime}^{k_s^{\prime}} + O_{(i,j,k,c,k_s^{\prime})\rightarrow(i,j^\prime,k^\prime,c^\prime,k_s^{\prime})})
    \end{multlined}
\label{eq:ilp-no-overlap}
\end{equation}

Equation~\ref{eq:ilp-no-overlap} adds a dependency constraint which specifies that two different operations cannot overlap in time if they are executed on the same worker.
For example, if operation $(i, j', k', c', k_s^\prime)$ is scheduled after $(i, j, k, c, k_s^\prime)$, they both execute on worker $(i, k_s^\prime)$ and thus $(i, j', k', c', k_s^\prime)$  must begin after $(i, j, k, c, k_s^\prime)$ ends.
\myzhao{I think the original $O$ ordering was the wrong way around so I flipped it, double check me.}

\noindent\textit{Memory Constraint.}
\begin{equation}
    \begin{multlined}
    M_{Limit} \ge \Delta M_{i,j^\prime,k^\prime,c^\prime}^{k_s^{\prime}} + \\ \sum_{j,k,c} \Delta M_{i,j,k,c}^{k_s^{\prime}} \times O_{(i,j,k,c,k_s^{\prime})\rightarrow(i,j^\prime,k^\prime,c^\prime,k_s^{\prime})}
    \end{multlined}
\label{eq:ilp-memory}
\end{equation}

Finally Equation~\ref{eq:ilp-memory} calculates the activation memory required at any given time on worker $(i, k_s^\prime)$, and constrains operations such that the total memory is below an $M_{limit}$ to avoid OOMs.

\noindent\textbf{Summary.}
The MILP above is formulated to capture and automatically leverage the key techniques described in Section~\ref{sec:system}.
By defining the notion of a \textit{surrogate} pipeline $k_s$, the MILP can express that $(i, j, k, c, k_s)$ schedules the original mini-batch intended for $k$ on $k_s$, implementing \textit{Adaptive Pipelines}.
Moreover, the range of $c$ contains $B_{weight}$ and $B_{input}$, allowing the MILP to separately schedule each, implementing \textit{Decoupled BackProp}.
Finally, \myzhao{@Swapnil, add a sentence on how the MILP can capture the staggered optimizer. I wasn't able to decipher that.}

Once the MILP outputs a solution, the \textit{Planner} simply converts the set of $O$ and $E$ variables (which explicitly specify pipeline operation orderings) into the optimal execution plan for the failure scenario to be used by \textit{Executors} as described in Section~\ref{sec:design_overview}.

\begin{comment}
\myzhao{===== OLD TEXT BELOW========}
\subsection{Inter-Group Fault Migration}

While \emph{adaptive pipelining} bolsters the resilience of hybrid parallel training jobs by ensuring training continues in face of one ore more failures, the loss of multiple data-parallel peers within the same pipeline stage can lead to uneven workload distribution across different data parallel groups, potentially creating bottlenecks that impede overall system performance. To mitigate this, \NAME may need to redistribute failure across data parallel peer groups, thus preventing any single group from becoming a bottleneck that limits throughput. Moreover, different stages of a pipeline have varying availability of ``bubbles'', and as \NAME leverages on these bubbles to minimize throughput loss, how failure are distributed across data parallel groups may have an impact on training throughput. 

To mitigate this challenge, we follow a dynamic programming (DP) approach to optimize the migration of tasks between data parallel groups. By effectively utilizing ``bubbles'' deeper in the pipeline where more bubbles are typically available, \NAME can minimize throughput loss and avoid performance bottlenecks, even when faced with multiple failures.

\paragraph{State}: Let \( dp[i][f] \) present the minimum overhead of handling \(f\) failures with \(i\) data parallel groups considered. Each stage has associated bubbles which are periods of idle time where no computations are occurring. 

\paragraph{Initial Condition}: Initialize \( dp[i][0] = 0 \), indicating that there is no cost when there are no failures to handle.

\paragraph{Recurrence Relation}: For each data parallel group \( i \) and \( f \) failures, update \( dp[i][f] \) by considering redistributing any number of failures \( x \) (where \( x \leq f \)) to the \( i^{th} \) group. The decision should account for the incremental use of bubbles and workload balancing:
\begin{equation}
    dp[i][f] = \argmin_{x \leq f}(dp[i-1][f-x] + \text{cost}(x, bubbles[i]))
\end{equation}
   
Here, ``cost'' is a function that calculates the impact of adding \( x \) failures' worth of micro batches to data parallel group \( i \).

\paragraph{Objective}: The goal is to minimize \( dp[F][N] \) where \( F \) is the total number of failures and \( PP \) is the total number of pipeline stages. This represents the minimum cost to allocate all failures optimally across the stages.

\paragraph{Complexity}: The complexity of this optimization procedure can be upper bounded by \(O(F \times PP^2)\), where \(F\) is the number of failures and \(PP\) is the depth of the pipeline. Empirically, we verify the optimization time with respect to the hybrid parallel strategy size in Table~\ref{???}.

\subsection{Adaptive Pipeline Computation Schedule}

While handcrafted schedules such 1F1B~\cite{pipedream} offer simplicity, they face several issues in practical applications. For one, scheduling under the assumption that \(T_B = 2 \times T_F\) introduces unwanted bubbles, especially for models where these values differ significantly. Moreover, communication time (denoted as \(T_{comm}\)) required to transfer activation/gradient between stages is often ignored in handcrafted schedules, leading to noticeable latencies in the pipeline stream~\cite{eager-1f1b}. Finally, striking a balance between minimizing bubble size and adhering to memory limit becomes particularly challenging when the available memory is insufficient, commonly the case with large scale training. To address these challenges and ensure generalization to practical scenarios, we formulate a Mixed Integer Linear Program (MILP), which can be solved by an off-the-shelf ILP solver, to automatically search for an optimal computation schedule given a parallelization strategy.

\subsubsection{MILP Formulation}\label{sec:ILP}

\paragraph{Inputs} We introduce \(T_{c}\) as the computational time for different phases \(c \in {Fm B_{Input}, B_{Weight}}\), and a binary mapping \(S_{i,j,k}^{k^\prime} \in \{ 0, 1 \}\) that indicates if a microbatch \( (j,k) \) at stage \(i\) is computed on pipeline \(k'\). Each computation phases for microbatch \( (j,k) \) at stage \(i\) is assigned to one and only one dataparallel pipeline i.e. \( \sum_{\substack{\hat{k}}} S_{i,j,k}^{\hat{k}} = 1 \). Finally, \(\Delta M_{i,j,k,c}^{k^\prime}\) takes into account the distinct memory requirements of different computational phases.

\begin{equation*}
\Delta M_{i,j,k,c}^{k^\prime} =
\begin{cases}
    A_{B} & \text{, if } c=F \text{ and  } S_{i,j,k}^{k^\prime} = 1 \\
    A_B - A_{B_{Input}} & \text{, if } c=B_{Input} \text{ and } S_{i,j,k}^{k^\prime} = 1 \\
    -A_{B_{Weight}} & \text{, if } c=B_{Weight} \text{ and } S_{i,j,k}^{k^\prime} = 1 \\
    0 & \text{, otherwise}
\end{cases}
\end{equation*}

Here, \(A_B\) is the size of activation stored at the end of forward pass, similarly \(A_{B_{Weight}}\) is size of activation stored at the end of backward-input pass. Upon completion of backward-input pass and backward-weight pass, we free activation \(A_{B_{Input}}\) and \(A_{B_{Weight}}\) respectively.

\paragraph{Variables} We want the MILP to search ordering of computation decisions in the schedule, for this we introduce variable \(O_{(i,j,k,c,\hat{k})\rightarrow(i^\prime,j^\prime,k^\prime,c^\prime,k^{\prime\prime})} \in \{ 0, 1 \}\), which indicates if compute decision \( (i,j,k,c,\hat{k}) \) is scheduled before \((i^\prime,j^\prime,k^\prime,c^\prime,k^{\prime\prime})\). Finally, we define \(E_{i,j,k,c}^{k^\prime}\) as the ending time of compute decision \( (i,j,k,c,k^\prime) \).

\paragraph{Optimization Target} Our primary goal is to minimize the makespan of training iterations by strategically sequencing the flow of micro batches through the training pipeline. This involves effectively managing sequential dependencies across various pipeline stages and computational phases, all while adhering to established memory constraints. We can formulate this goal as the following optimization problem:

\begin{equation}
    \min_{\substack{O, E}} \qquad \max_{\substack{i,j,k,k^\prime}} E_{i,j,k,W}^{k^\prime} 
\label{eq:ilp-optim-target}
\end{equation}

subject to

\paragraph{Cross-Stage Dependencies}
% Forward Pass
\begin{equation}
E_{i,j,k,F}^{k^\prime} \ge 
    S_{i,j,k}^{k^\prime} \times 
        (\sum_{\hat{k}} (E_{i-1,j,k,F}^{\hat{k}} \times S_{i-1,j,k}^{\hat{k}}) \\ + T_{comm} + T_{F})
\label{eq:ilp-cross-stage-dep-forward}
\end{equation}

% Backward-Input Pass
\begin{equation}
    \begin{multlined}
    E_{i,j,k,B_{Input}}^{k^\prime} \ge 
        S_{i,j,k}^{k^\prime} \times
            (\sum_{\hat{k}} (E_{i+1,j,k,B_{Input}}^{\hat{k}} \times S_{i+1,j,k}^{\hat{k}}) \\ + T_{comm} + T_{B_{Input}})
    \end{multlined}
\label{eq:ilp-cross-stage-dep-backward}
\end{equation}

\paragraph{Same-Stage Dependencies}
% Backward-Weight Pass
\begin{equation}
E_{i,j,k,B_{Weight}}^{k^\prime} \ge 
    S_{i,j,k}^{k^\prime} \times (E_{i,j,k,B_{Input}}^{k^\prime} + T_{B_{Weight}})
\label{eq:ilp-same-stage-dep}
\end{equation}

\paragraph{No-Overlapping computation decisions}
% Dependency imposed by our ordering constraint
\begin{equation}
    \begin{multlined}
    E_{i,j^\prime,k^{\prime},c^\prime}^{k^{\prime\prime}} \ge 
    E_{i,j,k,c}^{k^{\prime\prime}} + T_{c^\prime} - \\ \infty (1 - S_{i,j,k}^{k^{\prime\prime}} \times S_{i,j^\prime,k^\prime}^{k^{\prime\prime}} + O_{(i,j^\prime,k^\prime,c^\prime,k^{\prime\prime})\rightarrow(i,j,k,c,k^{\prime\prime})})
    \end{multlined}
\label{eq:ilp-no-overlap}
\end{equation}

\paragraph{Memory Constraints}
\begin{equation}
    \begin{multlined}
    M_{Limit} \ge \Delta M_{i,j^\prime,k^\prime,c^\prime}^{k^{\prime\prime}} + \\ \sum_{j,k,c} \Delta M_{i,j,k,c}^{k^{\prime\prime}} \times O_{(i,j,k,c,k^{\prime\prime})\rightarrow(i,j^\prime,k^\prime,c^\prime,k^{\prime\prime})}
    \end{multlined}
\label{eq:ilp-memory}
\end{equation}

Overall, constraints (\ref{eq:ilp-cross-stage-dep-forward}) and (\ref{eq:ilp-cross-stage-dep-backward}) add the sequential dependency requirements on the Forward and Backward passes of the same microbatch in adjacent pipeline stages, while constraint (\ref{eq:ilp-same-stage-dep}) adds dependency requirement between \(B_{Input}\) and \(B_{Weight}\) passes of the same microbatch in within a pipeline stage. Additionally, (\ref{eq:ilp-no-overlap}) adds the dependency constraint imposed by our decision of the scheduling order. Finally, (\ref{eq:ilp-memory}) limits the peak activations memory to be below \(M_{Limit}\).
\end{comment}

==> sections/runtime.tex <==
\section{\NAME Runtime}\label{sec:runtime}
\NAME consists of three primary components designed to optimize and execute distributed training processes:

\textbf{Planner}: Operating on CPUs, the planner explores optimization possibilities and crafts an execution plan. This module is responsible for intra-group distribution of micro batches and inter-group migration to ensure minimal throughput loss in face of one or more failures. Additionally, it also generates the computation schedule, striking a balance between minimizing bubble size and adhering to memory limit. The resulting execution plan is stored in a distributed instruction store, such as etcd, ready to be accessed by the Executors. 

\textbf{Execution plan}: Specifies micro batch assignment, pipeline execution schedule, and the communication order for each GPU. They are represented as sequences of \emph{pipeline instructions}, following the design principle of DeepSpeed~\cite{deepspeed}. The \emph{pipeline instructions} include \emph{ForwardPass}, \emph{BackwardPass}, which executes the forward/backward computation for a micro-batch. \emph{SendAct}, \emph{RecvAct}, \emph{SendGrad}, \emph{RecvGrad}, which sends/receives model activations/gradiendts. We further split \emph{BackwardPass} into \emph{BackwardInputPass} and \emph{BackwardWeightPass} to enable decoupled backprop. These \emph{pipeline instructions} are abstract key operations in hybrid-parallel training and allows for flexible pipeline scheduling and communication planning.

\textbf{Executor}: This module retrieves the execution plan from the instruction store and implements it on the GPUs according to the predefined schedule. It follows the pipeline instructions detailed in the plan, which include various operations essential for hybrid-parallel training: ForwardPass and BackwardPass (further divided into BackwardInputPass and BackwardWeightPass for decoupled backpropagation), as well as SendAct, RecvAct, SendGrad, and RecvGrad for managing data flows between computational nodes. These instructions, modeled on principles from DeepSpeed, ensure efficient computation and communication.

\textbf{Profiler}: Complementing the Planner, the profiler records execution times and memory usage, providing valuable data that the planner uses to create execution plan. This feedback loop is crucial for adjusting plans based on real-world performance metrics.
